Pruning Cannot Hurt Robustness: Certified Trade-offs in Reinforcement Learning

Reinforcement learning (RL) policies deployed in real-world environments must remain reliable under adversarial perturbations. At the same time, modern deep RL agents are heavily over-parameterized, raising costs and fragility concerns. While pruning has been shown to improve robustness in supervised learning, its role in adversarial RL remains poorly understood. We develop the first theoretical framework for certified robustness under pruning in state-adversarial Markov decision processes (SA-MDPs). For Gaussian and categorical policies with Lipschitz networks, we prove that element-wise pruning can only tighten certified robustness bounds; pruning never makes the policy less robust. Building on this, we derive a novel three-term regret decomposition that disentangles clean-task performance, pruning-induced performance loss, and robustness gains, exposing a fundamental performance--robustness frontier. Empirically, we evaluate magnitude and micro-pruning schedules on continuous-control benchmarks with strong policy-aware adversaries. Across tasks, pruning consistently uncovers reproducible ``sweet spots'' at moderate sparsity levels, where robustness improves substantially without harming - and sometimes even enhancing - clean performance. These results position pruning not merely as a compression tool but as a structural intervention for robust RL.

==> sections/5_experiment_setup.tex <==
% ================================================================
\section{Experimental setup}
\label{sec:exp}
% ================================================================
\textbf{Environments. }\label{sec:exp:envs}
We evaluate robustness in pruned victim networks against an trained adversary in two settings: classic continuous-control tasks from \texttt{MuJoCo} \cite{DBLP:conf/iros/TodorovET12}, and a symbolic, partially-observable grid world from \texttt{Craftax} \cite{DBLP:conf/icml/MatthewsBESJCF24}. For \texttt{MuJoCo}, we use the standard \texttt{Hopper} \cite{DBLP:conf/rss/ErezTT11} and \texttt{HalfCheetah} \cite{DBLP:conf/icannga/Wawrzynski09} tasks, where agents control locomotion using continuous-valued torques.
%
\texttt{Craftax-Symbolic-v1} is a challenging, procedurally generated 2D environment based on the Crafter benchmark \cite{DBLP:conf/iclr/Hafner22}. Each observation consists of a symbolic encoding of the agent’s $9\times11$ local view, including block types, nearby enemies, and internal state (e.g., health, hunger, inventory). The action space is discrete with 43 possible actions, and the environment tests long-term memory, planning, and exploration.

\textbf{Environment specific observation perturbations.}
To perturb \texttt{MuJoCo} observations (e.g., \texttt{Hopper} and \texttt{HalfCheetah}), we inject small, learnable noise into the agent's observation vector. Let $s_t \in \mathbb{R}^D$ denote the original state observation, where $D = 11$ for \texttt{Hopper} and $D = 17$ for \texttt{HalfCheetah}. Our adversarial network outputs the parameters of a diagonal Gaussian distribution. It maps $s_t$ to
\(
\mu_\theta(x) \in \mathbb{R}^D,  \log \sigma_\theta(x) \in \mathbb{R}^D,
\)
defining an element-wise independent Gaussian distribution over perturbations:
\(
\delta \sim \mathcal{N} \bigl( \mu_\theta(s_t),\, \mathrm{diag}(\sigma_\theta(s_t)^2) \bigr).
\)
To promote stealth, we regularize the $L_2$ norm $\|\delta\|_2$ and incorporate it into the adversarial PPO loss. We also include the log-probabilities of both $\delta$ and $m$ in the objective to maintain correct likelihood weighting during optimization.

For simplicity, when attacking \texttt{Craftax} states we only modify the blocks the agent can see on the map. However, care must be taken to create valid adversarial observations. The symbolic \texttt{Craftax} environment encodes blocks using a one hot encoding of $37$ block IDs. That is, for each tile in the agent's map view we have a vector of length $37$. The adversarial agent outputs a categorical distribution for each tile \(\mathrm{Categorical}(\boldsymbol{z}_{\theta}^i)\) where \(\boldsymbol{z}_{\theta}^i \) are the network logits for \(i \in \{1, \dots N_{tiles} (=99) \}\). Once the model has produced logits $\boldsymbol{z}_\theta^i$ for tile $i$, we sample a discrete block index
$
b^i \sim \mathrm{Categorical}\bigl(\boldsymbol{z}_\theta^i\bigr),b^i\in\{1,\dots,37\}.
$
We then convert this integer into a one–hot vector
$$
\mathbf{e}^i\in\{0,1\}^{37},\qquad
\mathbf{e}^i_k = 
\begin{cases}
1 & k = b^i,\\
0 & \text{otherwise},
\end{cases}
$$
and replace the original 37-dimensional encoding of tile $i$ with $\mathbf{e}^i$.  In this way every perturbed observation remains a valid \texttt{Craftax} state — each tile is still represented by exactly one active block ID — while allowing the adversary to inject learned, categorical “flips” into the map. We use the Hamming distance for our stealth norm.

As discussed in Section \ref{sec:method}, our adversarial network also outputs a Bernoulli mask. We specifically evaluate attack rates $r \in \{0.5, 1.0\}$. Furthermore, for \texttt{Hopper} and \texttt{HalfCheetah}, we evaluate our victim policies against adversaries with 10 logarithmically spaced $\lambda_{stealth}$ values between \(0.1\) and \(1000\); for \texttt{Craftax}, we do the same between \(0.01\) and \(10\) (we found larger values correspond to attacks that don't impact the victim policy). Additionally, adversaries are trained against an unpruned victim policies for each architecture and attack rate in \((\texttt{architecture}, r) \in \{\texttt{MLP}, \texttt{RNN}\} \times \{0.5, 1.0\}\). We detail the network architectures and hyperparameters for both the victims and adversaries networks in Appendix \ref{app:config}.

% ------------------------------------------------------------------
% ------------------------------------------------------------------
\textbf{Pruning method.}\label{sec:exp:pruning}
Instead of pruning a fully-trained network, we follow a linear iterative pruning \emph{schedule} throughout training, similar to \cite{DBLP:conf/eccv/HuangW18}. Every victim network is initialised \emph{dense}, with all its parameters.  We then remove parameters on-the-fly through training, linearly increasing the sparsity until some target is reached (removing $x\%$ of the parameters over the first $x\%$ of the training steps). No weight rewinding or fine-tuning is performed afterwards. We separately train models pruned to \textit{sparsities} of $50\,\%, 80\,\%,$ and $90\,\%$ for which parameter counts can be found in Appendix \ref{app:config}, Table \ref{tab:pruning}.



% Starting after an initial warm-up of $10\,\%$ of the total updates,
% we linearly increase the sparsity mask at each optimisation step until the
% target level is reached at one of $50\,\%, 80\,\%,$ and $90\,\%$ of training.
% No weight rewinding or fine-tuning is performed afterwards. Parameter counts of pruned models can be found in Appendix \ref{app:param_counts}.



% We consider three pruning \emph{types} (see \ref{sec:lit:pruning} for more information on pruning):
% \textbf{magnitude}, a deterministic global magnitude pruning;  
% \textbf{magnitude\_ste} - same mask, but gradients flow through zeros via a straight-through estimator;  
% \textbf{random} - fixed random mask with the same density.  

We consider three pruning algorithms to determine which parameters to remove:

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-2em}
    \setlength{\tabcolsep}{1pt}  % Reduce space between columns
    \centering
    % \begin{tabular}{p{0.01cm}ll}
    \begin{tabular}{p{0.23cm}cc}
        % \toprule
        & \small{Natural Observation} & \small{Adversarial Observation}\\
        % \midrule

        \rotatebox{90}{\small{Craftax-Symbolic}} & 
        \includegraphics[width=0.48\linewidth]{\imagepath craftax/normal/b.png} & 
        \includegraphics[width=0.48\linewidth]{\imagepath craftax/adversarial/b.png} \\
        
        \rotatebox{90}{\small{HalfCheetah}} & 
        \includegraphics[width=0.48\linewidth]{\imagepath halfcheetah/normal/a.png} & 
        \includegraphics[width=0.48\linewidth]{\imagepath halfcheetah/adversarial\advcircle /a.png} \\

        \rotatebox{90}{\small{Hopper}} &
        \includegraphics[width=0.48\linewidth]{\imagepath hopper/normal/b.png} & 
        \includegraphics[width=0.48\linewidth]{\imagepath hopper/adversarial\advcircle /b.png} \\
        % \bottomrule
    \end{tabular}
    \caption{Visualisations of natural observations and their corresponding (extreme) adversarial perturbations in the \texttt{MuJoCo} and \texttt{Craftax} environments, with changes highlighted in {\color{red}red}. For \texttt{Craftax}, the crafting table is replaced by a tree. Further examples can be found in Appendix \ref{app:perturbations}.}
    \label{fig:perturbation)_grid}
    \vspace{-7em}
\end{wrapfigure}

\textbf{Magnitude} \cite{DBLP:conf/nips/CunDS89} - deterministic global magnitude pruning, removing the smallest $x\%$ of parameters.

\textbf{Magnitude + STE} \cite{DBLP:conf/wacv/VanderschuerenV23} - the same algorithm as magnitude pruning, but with the inclusion of the Straight-Through Estimator (STE) \cite{DBLP:journals/corr/BengioLC13, Hinton2012Coursera} in backpropagation. This treats the non-differentiable mask as an identity operator, allowing gradients to flow through the pruned connections.

\textbf{Random} \cite{DBLP:conf/iclr/LiuCC0MWP22} - a naïve approach which selects $x\%$ of parameters to remove stochastically.

All algorithms are augmented with a Erdős–Rényi Kernel (ERK) \textit{distance metric}, as per \cite{DBLP:conf/iclr/LeePMAS21, DBLP:conf/icml/EvciGMCE20,  mocanu_scalable_2018}. This calculates a pruning scaling factor for each layer based on the number of parameters it has, making larger layers more sparse. 

Pruning is implemented with JaxPruner \cite{lee2024jaxpruner}. 

\textbf{Reproducibility.} All reported metrics are averaged over \textbf{4} training seeds. Error bars show the \emph{95\% confidence interval}, computed as $\pm1.96\,\mathrm{SEM}$. We evaluate performance of each pruning type vs adversary (of each architecture type) by playing $1000$ episodes which we average performance metrics across.



% \begin{itemize}[leftmargin=1.4em,itemsep=0.15em]
% \item \textbf{magnitude} - deterministic global magnitude pruning;  
% \item \textbf{magnitude\_ste} - same mask, but gradients flow through zeros via a straight-through estimator;  
% \item \textbf{random} - fixed random mask with the same density.  
% \end{itemize}
% ------------------------------------------------------------------







%\section{MOVE TO APPENDIX / BIN}
%Our study spans two families of benchmarks- \texttt{MuJoCo} %\cite{DBLP:conf/iros/TodorovET12} continuous-control tasks %and the partially-observable \texttf{Craftax} %\cite{DBLP:conf/icml/MatthewsBESJCF24} grid world.  
%Unless noted otherwise, all headline numbers are the mean %across \textbf{4} training seeds; error bars in all figures %show the \emph{95\% confidence interval} computed as
%$\pm1.96\,\mathrm{SEM}$.

% ------------------------------------------------------------------


%\noindent
%\begin{minipage}[t]{0.2\textwidth}
  %\vspace{-\baselineskip} % Removes the vertical gap at the %top
%  \centering
%  \includegraphics[width=\linewidth]{imgs/halfcheetah.png}
%  \captionof{figure}{\texttt{MuJoCo}}
%  \vspace{0.5em} % Small space between images
%  \includegraphics[width=\linewidth]{imgs/craftax.png}
%  \captionof{figure}{\texttt{Craftax}}
%\end{minipage}\hfill
%\begin{minipage}[t]{0.78\textwidth}
  %\vspace{-\baselineskip} % Match vertical alignment with the %left minipage

  %\subsection{Benchmarks and Victim %Policies}\label{sec:exp:envs}

  %\texttt{MuJoCo. }%\par
  %This is a widely adopted benchmark for reinforcement %learning, modelling continuous control of simulated robotic %movements under physical laws. 
  %We use the \texttt{Hopper} \cite{DBLP:conf/rss/ErezTT11} %and \texttt{HalfCheetah} %\cite{DBLP:conf/icannga/Wawrzynski09} environments which %respectively have action spaces of 3 and 6 real valued %variables corresponding to motor torque. Each is used at %the default 1 kHz control rate. 
  %Victim policies are trained with Proximal Policy %Optimisation (PPO) for
  %\mbox{50 M} environment transitions - approximately 40 M %parameter-updates with a horizon of
  %2048 steps.
    
 % \texttt{Craftax.}%\par
  % \textit{Craftax-Symbolic-v1} is a $9\times11$ partially-observable 3-D grid world. 
%This is an optimised Jax rewrite of the challenging Crafter %\cite{DBLP:conf/iclr/Hafner22} benchmark - we use the %\texttt{Craftax-Symbolic-v1} variant which provides a %partially-observable 2-D grid world. This procedurally %generated environment challenges RL agents in exploration, %planning, and long term memory. Each observation is a %symbolic encoding of local world features (block types, %enemies) and agent state (e.g., health, hunger, inventory) %and at each step an action is sampled from the space of 43 %possible discrete actions.
% \textit{Craftax-Symbolic-v1} is a $9\times11$ partially-observable 3-D grid world, a benchmark challenging reinforcement learning agents in exploration, planning, and memory within procedurally generated environments. Observations are symbolic, encoding local world features and agent status (e.g., health, inventory). The environment features a discrete action space, typically with 17 actions for this variant. Interactions are step-based, rather than following a fixed real-time control rate. Victims are trained with the same PPO implementation for 100 M transitions.
%Victims are trained with the same PPO implementation for 100 %M transitions.

%\end{minipage}

%For each environment we keep two architectural variants: %\textbf{MLP}: a feed-forward actor-critic baseline;
%\textbf{RNN}: the same network augmented with a gated-%recurrent layer,
%allowing the policy to exploit temporal information.
% \begin{itemize}[leftmargin=1.4em,itemsep=0.15em]
% \item \textbf{MLP}: a feed-forward actor-critic baseline.
% \item \textbf{RNN}: the same network augmented with a gated-recurrent layer,
%   allowing the policy to exploit temporal information.
% \end{itemize}
%All optimiser settings and network widths are identical %across dense and pruned models;
%full hyper-parameters appear in Appendix %~\ref{app:hyperparams}.



